Efficient Recommendation with Millions of Items by Dynamic Pruning of Sub-Item Embeddings

A large item catalogue is a major challenge for deploying modern sequential recommender models, since it makes the memory footprint of the model large and increases inference latency. One promising approach to address this is RecJPQ, which replaces item embeddings with sub-item embeddings. However, slow inference remains problematic because finding the top highest-scored items usually requires scoring all items in the catalogue, which may not be feasible for large catalogues. By adapting dynamic pruning concepts from document retrieval, we propose the RecJPQPrune dynamic pruning algorithm to efficiently find the top highest-scored items without computing the scores of all items in the catalogue. Our RecJPQPrune algorithm is safe-up-to-rank K since it theoretically guarantees that no potentially high-scored item is excluded from the final top K recommendation list, thereby ensuring no impact on effectiveness. Our experiments on two large datasets and three recommendation models demonstrate the efficiency achievable using RecJPQPrune: for instance, on the Tmall dataset with 2.2M items, we can reduce the median model scoring time by 64 times compared to the Transformer Default baseline, and 5.3 times compared to a recent scoring approach called PQTopK. Overall, this paper demonstrates the effective and efficient inference of Transformer-based recommendation models at catalogue scales not previously reported in the literature. Indeed, our RecJPQPrune algorithm can score 2 million items in under 10 milliseconds without GPUs, and without relying on Approximate Nearest Neighbour (ANN) techniques.

==> commented_recpqprune.tex <==
\begin{algorithm*}[b]
\small
\caption{\jpqprune{}($G$, $Inv$, $S$, $K$)}\label{alg:jpqprune_full}
\begin{algorithmic}[1]
   \Require $G$ is the codebook, defined by Eq.~\eqref{eq:sub_ids_map}
   \Require $Inv$ is the inverted index, mapping from sub-ids to items, as defined by Eq.~\eqref{eq:inverted_index}
   \Require $S$ is the matrix of pre-computed sub-item scores, indexed by split and sub-item, as per Eq.~\eqref{eq:sub_item_scores}  
   \Require $K$ is the number of results to return
    \State $sortedSubIds \gets$ sorted sub-ids in each split according to their score\label{alg:jpqprune:sort}

   \State $currentSubIds \gets$ array of size $m$ intialised with 1s \Comment{Unprocessed  sub-ids in $U_k$ are stored in  $sortedSubIds[k]$ starting from $currentSubIds[k]$} 

   \State $\sigma$ $\gets$ $\sum_{k=1}^{m} \text{$S[sortedSubIds[k][1]]$}$ \Comment{Score upper bound; as defined by Eq.~\eqref{eq:upper_bound_strict}}
   \State  $\theta \gets -\infty$  \Comment{Pruning threshold}
   \State $currentTopK$ $\gets$ None \Comment{list of current best $K$ <ItemId, score> pairs, sorted by score in decreasing order}
   \While{$\sigma$ > $\theta$} \Comment{Equation~\eqref{eq:pruning_condition}} \label{alg:jpqprune:mainloop}
        \State $bestSplit$ $\gets \argmax_{ 1 \leq \text{k} \leq m} S[k][sortedSubIds[currentSubIds[k]]]$ \Comment{Find highest-scored unprocessed $\langle$SplitId, SubId$\rangle$ pair} \label{alg:jpqprune:bestsplit}
        \State $bestSubId$ $\gets sortedSubIds[bestSplit][currentSubIds[bestSplit]]$
        \State $itemsToScore$ $\gets$ $Inv[bestSplit][bestSubId]$ \Comment{Retrieve all items associated with the $\langle$bestSplit, bestSubId$\rangle$} \label{alg:jpqprune:retr}
        \State $scoredTopK$ $\gets$ \texttt{PQTopK}($G$, $S$, $K$, $itemsToScore$) \Comment{Find top $K$ items, associated with $\langle bestSplit, bestSubId \rangle$ pair using Algorithm~\ref{alg:top_k}}\label{alg:jpqrune:score}
        \State $currentTopK$ $\gets$ \texttt{merge}($currentTopK$, $scoredTopK$, $K$) \Comment{Update top $K$ items. \texttt{merge} removes duplicates \& selects best $K$ $\langle$ItemId, score$\rangle$ pairs}  \label{alg:jpqprune:update_topk}
        \State $currentSubIds$[$bestSplit$]  $\gets$ $currentSubIds$[$bestSplit$] + 1 \Comment{Remove $\langle bestSplit$, $bestSubId \rangle$ from the unprocessed set $U$} \label{alg:jpqprune:remove}
        \State $\sigma$ $\gets$ $\sum_{k=1}^{m} S[k][sortedSubIds[k][currentSubIds[k]]]$ \Comment{Update upper bound using Eq.~\eqref{eq:upper_bound_strict}} \label{alg:jpqprune:update_ub}
        \State $\theta \gets$ $currentTopK$[$K$].score \Comment{New threshold is the score of the $K$-th best item} \label{alg:jpqprune:update_threshold}
   \EndWhile
   \State\Return $currentTopK$ 
\end{algorithmic}
\end{algorithm*}


==> old_alg.tex <==





\subsection{RecPQPrune Algorithm}\label{ssec:alg}

\begin{algorithm}[tb]
\inote{add batching to the alorithm}
\small
\caption{\jpqprune{}($G$, $Inv$, $S$, $K$)}\label{alg:jpqprune}
\begin{algorithmic}[1]
   \Require $G$ is the codebook, defined by Eq.~\eqref{eq:sub_ids_map}
   \Require $Inv$ is the inverted index, mapping from sub-ids to items, as defined by Eq.~\eqref{eq:inverted_index}
   \Require $S$ is the matrix of pre-computed sub-item scores, indexed by split and sub-item, as per Eq.~\eqref{eq:sub_item_scores}  
   \Require $K$ is the number of results to return
    \State $sortedSubIds \gets$ sorted sub-ids in each split according to their score\label{alg:jpqprune:sort}
   \Require \sg{$batchSize$ is the number of sub-ids processed at every iteration.}. 

   \State $currentSubIds \gets$ array of size $m$ intialised with 1s 

   \State $\sigma$ $\gets$ $\sum_{k=1}^{m} \text{$S[sortedSubIds[k][1]]$}$
   \State  $\theta \gets -\infty$  
   \State $currentTopK$ $\gets$ None 
   \While{$\sigma$ > $\theta$}  \label{alg:jpqprune:mainloop}
        \State $bestSplit$ $\gets \argmax_{ 1 \leq \text{k} \leq m} S[k][sortedSubIds[currentSubIds[k]]]$ \label{alg:jpqprune:bestsplit}
        \State $bestSubIds$ $\gets sortedSubIds[bestSplit][currentSubIds[bestSplit] : \sg{currentSubIds[bestSplit] + batchSize}]$
        \State $itemsToScore$ $\gets$ $\bigcup_{bestSubId \in BestSubIds} Inv[bestSplit][bestSubId]$  \label{alg:jpqprune:retr}
        \State $scoredTopK$ $\gets$ \texttt{PQTopK}($G$, $S$, $K$, $itemsToScore$) \label{alg:jpqrune:score}
        \State $currentTopK$ $\gets$ \texttt{merge}($currentTopK$, $scoredTopK$, $K$) \label{alg:jpqprune:update_topk}
        \State $currentSubIds$[$bestSplit$]  $\gets$ $currentSubIds$[$bestSplit$] + \sg{batchSize} \label{alg:jpqprune:remove}
        \State $\sigma$ $\gets$ $\sum_{k=1}^{m} S[k][sortedSubIds[k][currentSubIds[k]]]$  \label{alg:jpqprune:update_ub}
        \State $\theta \gets$ $currentTopK$[$K$].score  \label{alg:jpqprune:update_threshold}
   \EndWhile
   \State\Return $currentTopK$ 
\end{algorithmic}
\end{algorithm}

Using Principles P1 and P2, we can now derive the \jpqprune{} algorithm. Algorithm~\ref{alg:jpqprune} presents \jpqprune{} in the form of pseudo-code \rsasha{(we also include a version of the algorithm with detailed comments as Algorithm~\ref{alg:jpqprune_full} in auxiliary materials)}. 
According to Principle P1, \jpqprune{} processes sub-ids in the descending order of their scores. To achieve that, it sorts sub-ids according to their scores within each split (line~\ref{alg:jpqprune:sort}), and in each iteration, it finds the maximum-scored unprocessed sub-id, denoted as $bestSubId$ and corresponding split, denoted as $bestSplit$ (line~\ref{alg:jpqprune:bestsplit}). 

In order to be able to quickly score all items associated with the $\langle bestSplit$, $bestSubId \rangle$ \jpqprune{} uses an \emph{inverted index}, denoted $Inv$, that maps $\langle Split$, $Subid\rangle$ pairs to the set of all items associated with the pairs, i.e., an inversion of mapping $G$:
\begin{align}
Inv[k][j] = \left\{i^{kj}_1, i^{kj}_2 ... i^{kj}_n\right\} \; \text{such that}\; \forall a: G[i^{kj}_a][k] = j \label{eq:inverted_index}
\end{align}

\looseness -1 When processing $bestSubId$, \jpqprune{} retrieves all items associated with this sub-id from the inverted index $Inv$ (line~\ref{alg:jpqprune:retr}); computes scores of all items associated with this sub-id using the PQTopK algorithm (line~\ref{alg:jpqrune:score}); updates current best top $K$ items (line~\ref{alg:jpqprune:update_topk}).  Note that because every item is associated with multiple sub-ids, \jpqprune{} may score every item multiple times; therefore, when updating current best top $K$ items, \jpqprune{} also deduplicates any repeated items.  It then removes this sub-id from the unprocessed set (line~\ref{alg:jpqprune:remove}); updates the upper bound $\sigma$ (line~\ref{alg:jpqprune:update_ub}) and the pruning threshold $\theta$ (line~\ref{alg:jpqprune:update_threshold}). \jpqprune{} iterates until the pruning condition (Equation~\eqref{eq:pruning_condition}) is met, after which it terminates and returns the current best top $K$ items.


==> removed_bits.tex <==

\subsection{Unsafe \jpqprune{}}\label{ssec:unsafe}
\inote{Sasha: I'm tempted to remove Unsafe and submit it to the next venue after safe is accepted}

In initial experiments,  we found that \jpqprune{} identifies the exact top $K$ highest-scored item much earlier than the pruning condition would suggest. To mitigate this problem and further improve efficiency, we propose two unsafe modifications of \jpqprune{}, both of which modify the pruning condition (Equation~\eqref{eq:pruning_condition}). 

\paragraph{Modification 1: Limited processing of sub-ids} We can limit the maximum number of
processed sub-ids by changing the main loop condition  (line~\ref{alg:jpqprune:mainloop} of Algorithm~\ref{alg:jpqprune}) to:
\begin{align}
    (\sigma > \theta) \And (\textit{iteration} < \textit{maxIterations})
\end{align}
where variable \texttt{iteration} increases at every step of the loop, and \textit{maxIterations} is a hyperparameter that controls the effectiveness/effi\-ci\-ency tradeoff of the algorithm. As we show in Section~\ref{ssec:results_tradeoffs}, choosing the right value of \textit{maxIterations} can reduce the models' inference time by a large margin while only having a limited effect on effectiveness. Moreover, controlling the maximum number of iterations may be desirable for some deployment settings where there are Service Level Agreements in place for response times.

Limiting the number of terms (sub-ids) is also used in TAAT Quit~\cite{buckley:1985,Moffat94fastranking}, which provides our inspiration for this modification.

\paragraph{Modification 2: Inflated threshold} 
Broder et al.~\cite{10.1145/956863.956944} proposed an unsafe modification of WAND based on artificially inflating the threshold for scoring new documents. This inspires our alternative modification that allows \jpqprune{} to terminate earlier is based on the idea of relaxation of the pruning condition. In this modification, the main loop condition changes to:
\begin{align}
    \sigma > F\times\theta 
\end{align}
where $F>1$ is a threshold inflation hyperparameter. With larger $F$, the pruning condition is achieved faster\footnote{\rsasha{we assume that the threshold value $\theta$ is positive (otherwise multiplying it by the constant $F>1$ would decrease it instead of increasing); if both negative and positive scores are possible, a similar effect can be achieved for example by applying a logistic sigmoid transformation to both threshold and upper bound: $\text{sigmoid}(\sigma) > F\times\text{sigmoid}(\theta)$.}}. Compared to Modification~1, this modification does not provide any guarantees that the algorithm will stop after any specific number of iterations. However, we postulate that adjusting $F$ may provide more fine-grained control than the number of iterations. This is because some sequences may be hard to prune\footnote{For more on pruning difficulty in document retrieval, see \cite{10.1145/2348283.2348367,10.1145/2433396.2433407}.} (i.e.\ many items have similar scores, and hence the threshold does not rise quickly), while others can be easier to prune (sufficient highly scored items to allow rapid termination). Controlling $F$ to make more aggressive pruning is more likely to retain effectiveness for difficult sequences (by not stopping too early) compared to setting a low number of iterations.















\subsection{PQ for Recommender Systems \rsasha{and PQTopK}}\label{ssec:recjpq}
\inote{this is covered in the RecSys Short Paper}


\begin{figure}[tb]\hspace{-3mm}
    \vspace{-0.5\baselineskip}
\includegraphics[width=0.5\textwidth]{figures/pq_scoring_graffle.pdf}%
    \caption{Reconstruction of item embeddings \sasha{and computing item scores} using Product Quantisation \sasha{with $m=3$ splits.} }\vspace{-.75\baselineskip}
    \label{fig:embedding_reconstruction}
    
\end{figure}


As we noted above, with large item catalogues, the item embedding matrix $W$ requires too much memory to store. Indeed, when the catalogue size reaches several million items, the item embedding matrix becomes too large to fit in a GPU's memory~\cite{petrovRecJPQTrainingLargeCatalogue2024}. To reduce its memory footprint, several recent recommendation models adopted Product Quantisation (PQ)~\cite{jegouProductQuantizationNearest2011} -- a well-studied method for vector compression. PQ is a generic method that can be applied to any \nt{set of vectors}; however, in this section, we \nt{describe} PQ as applied to item embedding. %




\looseness -1 To compress the item embedding matrix $W$, PQ associates each item id to a list of {\em sub-ids}, akin to language models breaking down words into sub-word tokens. PQ reconstructs an item's embedding by combining the sub-id embeddings assigned to it. These sub-ids are organised into {\em splits}, with each item having precisely one sub-id from each split\footnote{We use the terminology from~\cite{petrovRecJPQTrainingLargeCatalogue2024}. In the PQ literature, another popular term for sub-id embeddings is \emph{centroids}, and another popular term for splits is \emph{sub-spaces}.}. More formally, PQ first builds a \emph{codebook} $G\in\mathbb{N}^{|I|\times m}$ that maps an item id $i$ to its associated $m$ sub-ids:
\begin{align}
    G[i] \rightarrow \left\{g_{i1}, g_{i2}, ..., g_{im}\right\} \label{eq:sub_ids_map}
\end{align}
where $g_{ij}$ is the $j$-th sub-id associated with item $i$ and $m$ is the number of splits. To achieve compression compared to storing a full item embedding matrix, $m$ is typically chosen much smaller compared to full embeddings dimensionality: $m \ll d$.
The exact algorithm for associating ids with sub-ids is specific to different implementations of PQ. For example, the original PQ implementation uses variations of K-Means clustering, Differentiable Product Quantisation proposes a method to learn the mapping~\cite{chenDifferentiableProductQuantization2020} as part of overall model training, and RecJPQ~\cite{petrovRecJPQTrainingLargeCatalogue2024} derives the codes from a truncated SVD decomposition of the user-item interactions matrix. 


For each split $k=1,\ldots,m$, PQ stores a sub-item embedding matrix $\Psi_k \in \mathbb{R}^{b\times\frac{d}{m}}$, where $b$ is the number of distinct sub-ids in each split. The $j$-th row of $\Psi_k$ denotes the sub-item embedding $\psi_{k,j} \in \mathbb{R}^{\frac{d}{m}}$ associated with the $j$-th sub-id, in the $k$-th split.
Then, PQ reconstructs the item embedding $w_i$ as a concatenation of the associated sub-id embedding: 
\begin{align}
    w_i =  \psi_{1,g_{i1}} \mathbin\Vert \psi_{2,g_{i2}}  \mathbin\Vert ... \mathbin\Vert  \psi_{m,g_{im}} \label{eq:pq:item_embedding}
\end{align}

Finally, an item score is computed as the dot product of the  sequence embedding and the constructed item embedding: 
\begin{align}
    r_i = w_i \cdot \phi\label{eq:dot_product}
\end{align}

\looseness -1 A straightforward use of Equation~\eqref{eq:dot_product} for item scoring in PQ-based recommendation models does not lead to any computational efficiency improvements compared to models where all item embeddings are stored explicitly.
However, PQ offers a more efficient scoring algorithm, which serves as both a baseline and a backbone to \jpqprune{}. To achieve more efficient scoring, PQ  first splits the sequence embedding $\phi \in \mathbb{R}^{d}$ into $m$ sub-embeddings $\left\{\phi_1, \phi_2 ... \phi_m\right\}$, with $\phi_{k} \in \mathbb{R}^{\frac{d}{m}}$ for $k=1, \ldots,m$, such that $\phi = \phi_1  \mathbin\Vert \phi_2  \mathbin\Vert ... \mathbin\Vert  \phi_m$.
By substituting Equation~\eqref{eq:pq:item_embedding} and the similarly decomposed sequence embedding $\phi$ into Equation~\eqref{eq:dot_product}, we can compute the final item score for item $i$ as the sum of sub-embedding dot-products: 
\begin{align}
   r_i = w_i \cdot \phi &= (\psi_{1,g_{i1}} \mathbin\Vert ... \mathbin\Vert  \psi_{m,g_{im}}) \cdot (\phi_1  \mathbin\Vert ... \mathbin\Vert  \phi_m) = \sum_{k=1}^m \psi_{k,g_{ik}} \cdot \phi_k \nonumber
\end{align}

Let $S \in \mathbb{R}^{m \times b}$ denote the \emph{sub-id score matrix}, which consists of \emph{sub-id scores} $s_{k,j}$, defined as dot products of the sub-item embedding $\psi_{k,j}$ and the sequence sub-embeddings $\phi_k$:
\begin{align}
s_{k,j} = \psi_{k,j} \cdot \phi_k\label{eq:sub_item_scores}
\end{align}

The final score of item $i$ is then can be computed as the sum of the scores of its associated sub-ids:
\begin{align}
   r_{i} = \sum_{k=1}^m s_{k,g_{ik}} \label{eq:sum_sub_scores}
\end{align}

The number of splits $m$ and the number of sub-ids per spit $b$ are usually  chosen to be relatively small, 
so that the total number of sub-id scores is much less compared to the size of the catalogue, e.g., $m\times b \ll |I|$. 
Therefore,  we can pre-compute matrix $S$ \sasha{for a given sequence embedding} once and then reuse these scores for all items. This leads to efficiency gains compared to matrix multiplication, as scoring each item now only requires $m \ll d$ additions instead of $d$ multiplications and $d$ additions per item (Equation~\eqref{eq:scores}). The time for pre-computing sub-item scores matrix $S$ does not depend on the catalogue size $|I|$, and %
we can assume that it is negligible compared to exhaustive scoring of all items. 

\rsasha{In the paper, we refer to the summation-based approach as \textit{PQTopK}; we also include a pseudo-code version of the PQTopK as Algorithm~\ref{alg:top_k} \rsasha{in Auxiliary Materials}. \rsasha{PQTopK} allows selecting} top $K$ items not only from all items but from a specific subset of items -- we will use this feature of the algorithm later in \jpqprune{}.\footnote{In document retrieval parlance, this is a DAAT scoring algorithm, but operating using the direct index ($G$), rather than an inverted index.}

   


\looseness -1 While Algorithm~\ref{alg:top_k} is more efficient than matrix multiplication, it still requires the exhaustive scoring of every item in the catalogue, which is impractical for large catalogue deployments. However, as we show in the next section, the fact that item embeddings are constructed from shared sub-embeddings in PQ-based recommendation models allows the use of a novel pruning technique, which allows us to find the top $K$ items exactly without exhaustive scoring.%

\begin{figure}[tb]
\centering
\caption{Relation between item ranks and sub-item scores for user 82082 in Gowalla Dataset. The plot is based on the SASRec-RecJPQ model~\cite{petrovRecJPQTrainingLargeCatalogue2024} with 8 splits and 256 sub-ids per split. The top-ranked item is the item with the highest score (rank 1), the middle-ranked item is the item at rank 600,000 (out of 1.2M), and the bottom-ranked item is the item with the lowest score.} \label{fig:gowalla_heatmap}
\resizebox{ \linewidth}{!}{
    \includegraphics{figures/gowalla_heatmaps/user_82082.pdf}
}\vspace{-1.2em}
\end{figure}



\begin{table}[tb]
\caption{Effectiveness and \nt{median response times (mRT, in ms)} of different inference methods.  * denotes a statistically significant difference in NDCG@10 compared with the default matrix multiplication scoring ($p < 0.05$, Bonferroni multi-test correction). $^{\dagger}$ FAISS\texttt{.search()} call does not return the number of scored items.}    %
\label{tb:results_table}
\resizebox{\linewidth}{!}{
    \input{tables/main_table.tex}
}
\end{table}

Hence, we choose both the classical PQ in a popular library and the most recent implementation of PQ tailored to recommendation. To ensure a fair comparison, for both FAISS-based PQ and RecJPQ, we use a number of splits $m=8$ and the number of sub-ids per split $b=256$, as suggested in the RecJPQ paper~\cite{petrovRecJPQTrainingLargeCatalogue2024}.

For FAISS, we use the \texttt{.search()} method provided by the library. This method is applied to the same FAISS's PQ index as we use in other experiments.   Note that FAISS's \texttt{.search()} is an approximate nearest neighbour algorithm, which is not safe-to-rank $K$. Indeed, when we apply a safe version of \jpqprune{} to the FAISS index, we obtain better effectiveness than using \texttt{.search()} (see also Table~\ref{tb:results_table}). Finally, we omit any two-stage-based retrieval architectures, as any such architecture typically requires exhaustive scoring to identify candidate items for re-ranking.

\looseness -1 For effectiveness, we measure NDCG@10; statistically significant differences are measured using a paired-t test ($p<0.05$) with Bonferroni multiple testing test correction.
Following best practices, we do not apply negative sampling when computing any metrics~\cite{kricheneSampledMetricsItem2022, canamaresTargetItemSampling2020}. 




\subsection{\ref{rq:efficiency} Effect of \jpqprune{} on Inference Efficiency and Effectiveness}\label{ssec:rq1}



We first analyse the effectiveness and efficiency of \jpqprune{} compared to the baseline scoring methods, all based on the SASRec recommender model. Table~\ref{tb:results_table} reports the evaluation results of variations of our \jpqprune{} method compared to baseline methods on the two experimental datasets, Booking and Gowalla. We apply both FAISS-based PQ and RecJPQ for PQ-based item representation. We report measures for both effectiveness (NDCG@10) and efficiency (number of scored items and median response times).

\looseness -1 On analysing the table, we observe that the default SASRec item scoring method as defined by Equation~\eqref{eq:scores} (matrix multiplication) is by far the slowest. %
Indeed, on both datasets, the default SASRec's response time is dominated by the matrix multiplication, reaching 96\% of the overall response time on the larger-scale Gowalla dataset (406ms out of 424ms).
In contrast, the more efficient baseline scoring methods (FAISS.\texttt{search()} and RecJPQ with default PQTopK) require much less time for scoring. For example, on the smaller Booking dataset, both baselines achieve sub-millisecond response time (compared to 39ms required by the default scoring algorithm).  However, FAISS drops NDCG@10  by 55\% compared to full scoring (from 0.1352 to 0.0606), which arguably makes it impractical in real-life scenarios. The poor effectiveness of FAISS\texttt{.search()} is even more pronounced for the large Gowalla dataset, where NDCG@10 drops by 94\% compared to the default matrix multiplication approach. This poor performance of default FAISS's Product Quantisation echoes previous results in document retrieval~\cite{zhanJointlyOptimizingQuery2021}; the root cause of this drop is that the vector reconstruction objective (L2 metric) used by FAISS for PQ is not aligned with the ranking objective of the model. In contrast, RecJPQ integrates PQ into the model itself, improving efficiency without significantly damaging effectiveness. For example, on the Booking dataset, RecJPQ actually improves the effectiveness of default SASRec %
and on Gowalla, RecJPQ's NDCG is lower, but not by a statistically significant margin (0.1470 vs.\ 0.1372). 

When analysing the effectiveness and efficiency of \jpqprune{}, we first observe that the safe version of the algorithm applied to RecJPQ's PQ achieves exactly the same NDCG@10 as the default PQTopK applied to RecJPQ -- this provides empirical evidence for the fact that \jpqprune{} is safe-to-rank $K$. Moreover, on both datasets, when used with RecJPQ, the safe version of \jpqprune{} scores much fewer items compared to the exhaustive scoring of default (matrix multiplication) and PQTopK -- e.g.\ 2064 vs.\ 32958\footnote{Discrepancies between the number of processed items for exhaustive scoring compared with the catalogue size of the dataset are caused by the fact that some items were only present in validation or test splits of the dataset.} (-94\%) on Booking and 140476 vs.\ 1261640 (-89\%) on Gowalla. However, on Booking, \jpqprune{} does not lead to response time improvements -- the simplicity of the PQTopK algorithm (e.g.\ no extra function calls inside of the algorithm) allows it to be slightly faster compared to \jpqprune{}. In contrast, we see that on the larger Gowalla dataset, a smaller number of items processed by \jpqprune{} outweighs the overhead caused by extra complexity, and \jpqprune{} therefore improves median response time from 10.34ms to 8.61ms (-17\%). Notably, RecJPQ-based  RecPQPrune improves median response time (excluding the Transformer call) by 98\% with no significant difference in NDCG@10 w.r.t.\ SASRec's matrix multiplication.

We also observe from Table~\ref{tb:results_table} that unsafe versions of \jpqprune{} can further improve efficiency with only a moderate negative effect on effectiveness. For example, on the Gowalla dataset, the RecJPQ-based version of \jpqprune{} with a threshold inflated by 40\% allows for further reduction of the number of scored items compared to the safe version (39432 vs.\ 140476, -71\%) and response time (2.98ms vs.\ 8.61ms, -65\%). We further investigate efficiency/effective\-ness tradeoffs of unsafe modifications of \jpqprune{} in Section~\ref{ssec:results_tradeoffs}. 

Note that when applied to FAISS-based PQ, a safe version of \jpqprune{} scores \emph{more} items than exhaustive search. This is due to the fact that \jpqprune{} scores all items associated with a single sub-id; therefore, it can score an item multiple times. Due to the overall ineffectiveness of FAISS-based PQ, many items are scored multiple times before the pruning condition~Equation\eqref{eq:pruning_condition} allows scoring to terminate. However, unsafe modifications still allow for reducing the overall number of processed items. For example, on the Booking dataset, \sasha{unsafe \jpqprune{} with inflated threshold} applied to FAISS-based PQ reduces the number of scored items from 32958 to 16960 compared to exhaustive scoring. %

\looseness -1 In summary, we find that when a safe version \jpqprune{} is used with RecJPQ, it allows the reduction of the number of scored items by a large factor with no significant drop in effectiveness compared to both matrix multiplication and PQTopK-based scoring. On the Booking datasets, where the number of items is relatively small, this does not lead to improved response times compared to PQTopK, as the simplicity of PQTopK already allows sub-millisecond scoring. However, when the number of items in the catalogue is large, \jpqprune{} also leads to improved latency compared to PQTopK. We also found FAISS-based Product Quantisation to be ineffective for model inference, as the model training process is not aware of Product Quantisation in this case. Therefore, we exclude it from further analysis in RQ2 and RQ3 and focus on RecJPQ-based product quantisation moving forward.
Overall, in answer to RQ1, we find that when used with the effective RecJPQ method, \jpqprune{} always reduces the number of processed items compared to exhaustive scoring. When the number of items in the catalogue is large (c.f.\ Gowalla), this leads to reduced median response time.

\subsection{\ref{rq:cutoff} Effect of ranking cutoff $K$ on \jpqprune{}'s Efficiency and Effectiveness}\label{ssec:result_cutoff}
\begin{figure}
    \centering
    \subfloat[Effect on efficiency]{
        \includegraphics[width=0.48\linewidth]{figures/top_k_mrt.pdf} \label{fig:k_efficiency}
    }
    \subfloat[Effect on NDCG] {
        \includegraphics[width=0.48\linewidth]{figures/top_k_ndcg.pdf} \label{fig:k_ndcg}
    }
    \caption{\looseness -1 Effect of ranking cutoff $K$ on \jpqprune{}'s efficiency and effectiveness when applied to RecJPQ on the Gowalla dataset.  The baseline applies exhaustive scoring using the PQTopK algorithm. "Inflated Threshold" is an unsafe modification of \jpqprune{} with $F=1.4$. "Limited Iterations" is an unsafe modification of \jpqprune{} with the number of iterations limited to 8. \sasha{Reported time excludes inference of the backbone SASRec model.}}
    \label{fig:result_cutoff}\vspace{-1em}
\end{figure}

\looseness -1 The pruning condition (Equation~\eqref{eq:pruning_condition}) of \jpqprune{} depends on the threshold~$\theta$. %
Larger values of $K$ lead to smaller values of $\theta$, therefore reducing the efficiency of \jpqprune{}. Hence, we experimentally analyse the effect of ranking cutoff $K$ on the effectiveness and efficiency of \jpqprune{} when applied to RecJPQ on the Gowalla dataset. 
Of note, for effectiveness, we report NDCG@K while varying $K$ -- this avoids unfair comparisons when retrieving fewer items than the NDCG cutoff. We also omit the reporting of FAISS-based PQ methods, as well as the inefficient matrix multiplication baseline and the ineffective FAISS\texttt{.search()}.
\inote{Sasha: I think we should remove FAISS. It raises more questions than adds value. Noone asked a single question about FAISS in RecSys Reviews.}
Figure~\ref{fig:k_efficiency} shows the efficiency of different versions of \jpqprune{} when varying the cutoff $K$. As we can see, all safe and unsafe versions of \jpqprune{} are the most efficient for low-ranking cutoffs. For example, if we are only interested in a single top-scored item ($K=1$), the time required by the safe version of \jpqprune{} is just 3.07ms, which is 66\% less time compared to the baseline exhaustive scoring (PQTopK). In contrast, at higher cutoffs, safe \jpqprune{} becomes less efficient than exhaustive scoring. For example, with $K=64$, it requires 14.06ms, which is 28\% longer than exhaustive scoring. However, unsafe \jpqprune{} remains efficient even at high cutoffs $K$; for example, at the same cutoff $K=64$, the unsafe modification of \jpqprune{} using the threshold inflated by 40\% requires only 5.69ms (-47\% compared to the baseline) while the version with the number of iterations limited by 8 requires only 3.29ms. From Figure~\ref{fig:k_ndcg}, we see that these modifications only moderately reduce the effectiveness of the model at high cutoffs. For example, at ranking cutoff $K=64$, \sasha{the unsafe \jpqprune{} using inflated thresholds is only 1.2\% less effective than the safe setting (NDCG@64 0.1427 vs.\ 0.1445)}. %

Overall, it is clear that deployments of \jpqprune{} can further enhance efficiency compared to PQTopK by reducing the number of items retrieved or using unsafe modifications. Indeed, while the threshold inflation modification is marginally slower than limited iterations, it results in higher effectiveness across various rank cutoffs $K$. On the other hand, if scores are required for deep cutoffs, then \jpqprune{} is unnecessary.

\begin{figure}[tb]
    \centering
    \resizebox{0.9\linewidth}{!}{
        \includegraphics[width=\linewidth]{figures/tradeoffs.pdf} 
    }
    \caption{Effectiveness/Efficiency tradeoffs in the unsafe versions of \jpqprune{}, on the Gowalla dataset. 
    \sasha{Reported time excludes inference of the backbone SASRec model. *denotes statistically significant difference in NDCG compared to PQTopK ($p < 0.05$, Bonferroni multi-test correction).}}
    \label{fig:results_tradeoffs}\vspace{-1em}
\end{figure}



\subsection{\ref{rq:unsafe_tradeoffs} Effect of Unsafe Hyperparameters on  Effectiveness/Efficiency Tradeoff} \label{ssec:results_tradeoffs}

\looseness -1 We now consider the tradeoff between effectiveness and efficiency. Figure~\ref{fig:results_tradeoffs} presents a tradeoff graph allowing the comparison of effectiveness and efficiency. We fix $K=10$, as per Section~\ref{ssec:rq1}.
The default baseline (matrix multiplication), PQTopK and the safe version of \jpqprune{} are shown as points; the two unsafe modifications -- inflated threshold and max iterations -- are presented as curves. More desirable configurations are more effective with low response time (i.e.\ towards the top left-hand corner). Compared to the baseline and \jpqprune{}, it is possible to markedly reduce response time without a marked negative impact on effectiveness. For instance, \sasha{with $F=1.2$, NDCG@10 falls only by 0.4\% (0.1372  vs.\ 0.1366, not significant), but scoring time falls by 42\% (10.34ms vs.\ 6.05ms)}.  In general, we see that both modifications provide similar effectiveness/efficiency tradeoffs; however, the  Inflated Threshold modification achieves slightly higher NDCG values when the median response time is less than 4ms. Overall, in answer to RQ3, we find that both unsafe methods allow for a large reduction of response time with only a moderate negative impact on effectiveness when their parameters are selected appropriately. 




\begin{table}[tb]
\caption{Effectiveness and \nt{median response times (mRT, in ms)} of different inference methods, using BERT4Rec backbone.  * denotes a statistically significant difference in NDCG@10 compared with the default matrix multiplication scoring ($p < 0.05$, Bonferroni multi-test correction). $^{\dagger}$ FAISS\texttt{.search()} call does not return the number of scored items.}  \label{tb:results_table_gbert}
\resizebox{\linewidth}{!}{
    \input{tables/main_table_gbert.tex}
}
\end{table}



\looseness -1 Compared to existing methods for recommender systems with large catalogues, such as Approximate Nearest Neighbours (ANNs)~\cite{fredericksonApproximateNearestNeighbours2017, kelenProbabilisticPerspectiveNearest2021, chenApproximateNearestNeighbor2022} and two-stage ranking~\cite{hronComponentInteractionsTwoStage2021, maOffpolicyLearningTwostage2020}, \jpqprune{} is a \emph{safe-to-rank $K$} method, meaning that it provides theoretical guarantees that no highly-scored item is excluded from the top $K$ scored items. %
However, we also propose two \emph{unsafe} modifications of \jpqprune{}, which allow further reduction of the number of scored items with only a moderate impact on the model effectiveness. Moreover, compared to existing methods, \jpqprune{} is simpler, as it avoids training the first-stage candidate selection model as in 2-stage methods or reconstructing the full embedding tensor required for building the ANN index \sasha{(assuming that PQ is already part of the model)}. Overall, the contributions of this paper can be summarised as follows: (1) We propose \jpqprune{}, a safe and efficient method for sequential recommendation scoring, which is, to the best of our knowledge, the first adaptation of pruning-based methods to recommender systems; (2)  we propose \sasha{two unsafe modifications} of \jpqprune{}, which further improve scoring efficiency with only a moderate effect on model effectiveness; (3) we demonstrate the efficiency of \jpqprune{} through an extensive evaluation using \sasha{two} sequential recommendation datasets. 
For example, on Gowalla, when using the unsafe \jpqprune{}, we are able to reduce scoring time by 65\% compared to the safe modification while only moderately reducing NDCG@10 from 0.1372 to 0.1319. \inote{update}




==> rubbish.tex <==
Algorithm~\ref{alg:MaxScore} provides a high-level sketch of MaxScore DAAT Pruning. At each iteration, the algorithm finds the next promising document from the collection, computes its relevance score, and then updates \texttt{scoreUpperBound}. While details of \texttt{scoreUpperBound} computation are out of the scope of this paper, the main idea is that the algorithm guarantees that \emph{no unprocessed document can be scored higher than \texttt{scoreUpperBound}}. The algorithm also maintains $\theta$ -- the minimum score within current top-$k$ highest scored documents. 
When the algorithm already processed at least $k$ documents and \texttt{scoreUpperBound} $\le$ \texttt{$\theta$}, this means that (i) the algorithm already found $k$ documents with the score at least $\theta$ and (ii) no future unscored document will be higher than \texttt{$\theta$}; therefore it is guaranteed that the algorithm found top-$k$ exactly. 

\begin{algorithm}
\small
\caption{MaxScore DAAT Pruning}\label{alg:MaxScore}
\begin{algorithmic}
\Require $q$ \Comment{query}
\Require $\mathcal{D}$ \Comment {Documents collection}
\Require $k$ \Comment{Number of documents to return}
\State $d$ = nextMostPromisingDocid($q$, $D$) 
\State scoreUpperBound $\gets +\infty$
\State $\theta$ $\gets -\infty$
\State result $\gets $ A max-heap of at most $k$  
$\langle\text{docid}, \text{score}\rangle$ pairs
\While{(result.size() < $K$) \textbf{or} (upperBound < $\theta$)}
    \State score = $\sum_{t\in q} w(t,d)$ \Comment{fully score document $d$ using Eq.~\eqref{eq:ir_doc_score}}
    \State result.push($\langle$d, score$\rangle$)
    \State $\theta$ $\gets$ result.minScore()
    \State scoreUpperBound $\gets$ updateUpperBound($d$, $score$, $q$) 
    \State $d$ = nextMostPromisingDocid($q$, $D$)
\EndWhile
\State \Return result
\end{algorithmic}
\end{algorithm}

Revisiting the MaxScore Dynamic Pruning algorithm sketch (Algorithm~\ref{alg:MaxScore}), we find that to adapt this sketch for product-quantised recommender models, we have to figure out: 

\begin{enumerate}
    \item How to iterate over items so that the most promising items are likely to be scored first (i.e.\ define "nextMostPromisingDocid" in Algorithm~\ref{alg:MaxScore})
    \item How to define \texttt{scoreUpperBound} (i.e.\ guarantee that no future item will be scored higher than \texttt{scoreUpperBound})
\end{enumerate}



We now briefly analyse both items. 
\paragraph{Promising items order} Our approach to finding the most promising items (i.e. process items in such order that top-scored items are more likely to be processed first) is based on a hypothesis that \emph{if an item has a high score, its sub-items are also likely to have high scores}. Figure~\ref{fig:gowalla_heatmap} provides anecdotal evidence for the hypothesis. 




==> tables/main_table.tex <==
\begin{tabular}{l|ccc|ccccc}
\toprule
 Dataset$\rightarrow$ & \multicolumn{3}{r}{\makecell[c]{Booking}} & \multicolumn{3}{r}{\makecell[c]{Gowalla}} \\
Scoring type$\downarrow$  & \makecell[c]{NDCG\\@10} & \makecell[c]{Scored\\(median)} & \makecell[c]{mRT} & \makecell[c]{NDCG\\@10} & \makecell[c]{Scored\\(median)} & \makecell[c]{mRT} \\
\midrule\multicolumn{7}{c}{\textbf{Baselines}}\\\midrule

 Default & 0.135 & 32958 & 39.65 & 0.147 & 1261640 & 406.05 \\
 FAISS\texttt{.search()} & 0.061* & N/A$^{\dagger}$ & 0.33 & 0.008* & N/A$^{\dagger}$ & 4.10 \\
 RecJPQ+PQTopK & 0.192* & 32958 & 0.59 & 0.137 & 1261640 & 10.34 \\
\midrule\multicolumn{7}{c}{\textbf{RecPQPRune (FAISS-Based)}}\\\midrule

 Safe & 0.067* & 57240 & 3.40 & 0.008* & 2109904 & 40.95 \\
 Threshold inflated by 40\% & 0.068* & 10600 & 1.48 & 0.008* & 1520372 & 30.07 \\
 Max. 8 Iterations & 0.070* & 16960 & 1.36 & 0.005* & 124112 & 4.27 \\
\midrule\multicolumn{7}{c}{\textbf{RecPQPRune (RecJPQ-Based)}}\\\midrule

 Safe & 0.192* & 2064 & 1.54 & 0.137 & 140476 & 8.61 \\
 Threshold inflated by 40\% & 0.192* & 774 & 1.16 & 0.132* & 39432 & 2.98 \\
 Max. 8 Iterations & 0.192* & 1032 & 1.57 & 0.126* & 39432 & 2.55 \\
\bottomrule
\end{tabular}


==> tables/main_table_gbert.tex <==
\begin{tabular}{l|ccc|ccc}
\toprule
 Dataset$\rightarrow$ & \multicolumn{3}{r}{\makecell[c]{Booking}} & \multicolumn{3}{r}{\makecell[c]{Gowalla}} \\
Scoring type$\downarrow$  & \makecell[c]{NDCG\\@10} & \makecell[c]{Scored\\(median)} & \makecell[c]{mRT} & \makecell[c]{NDCG\\@10} & \makecell[c]{Scored\\(median)} & \makecell[c]{mRT} \\
\midrule\multicolumn{7}{c}{\textbf{Baselines}}\\\midrule

 Default & 0.253 & 32958 & 38.50 & 0.149 & 1261640 & 401.77 \\
 FAISS\texttt{.search()} & 0.158* & N/A$^{\dagger}$ & 0.34 & 0.066* & N/A$^{\dagger}$ & 4.15 \\
 RecJPQ+PQTopK & 0.332* & 32958 & 0.60 & 0.191* & 1261640 & 9.90 \\
\midrule\multicolumn{7}{c}{\textbf{RecPQPRune (FAISS-Based)}}\\\midrule

 Safe & 0.169* & 2328 & 1.21 & 0.066* & 2360743 & 70.98 \\
 Threshold inflated by 40\% & 0.169* & 1164 & 1.02 & 0.066* & 2117610 & 65.93 \\
 Max. 8 Iterations & 0.163* & 2328 & 1.48 & 0.065* & 62744 & 3.38 \\
\midrule\multicolumn{7}{c}{\textbf{RecPQPRune (RecJPQ-Based)}}\\\midrule

 Safe & 0.332* & 10449 & 4.57 & 0.191* & 118296 & 7.55 \\
 Threshold inflated by 40\% & 0.332* & 1806 & 1.26 & 0.191* & 69006 & 4.74 \\
 Max. 8 Iterations & 0.309* & 1032 & 1.77 & 0.179* & 39432 & 6.33 \\
\bottomrule
\end{tabular}

